Adaptively-Realistic Image Generation from Stroke and Sketch with Diffusion Model

Generating images from hand-drawings is a crucial and fundamental task in content creation. The translation is difficult as there exist infinite possibilities and the different users usually expect different outcomes. Therefore, we propose a unified framework supporting a three-dimensional control over the image synthesis from sketches and strokes based on diffusion models. Users can not only decide the level of faithfulness to the input strokes and sketches, but also the degree of realism, as the user inputs are usually not consistent with the real images. Qualitative and quantitative experiments demonstrate that our framework achieves state-of-the-art performance while providing flexibility in generating customized images with control over shape, color, and realism. Moreover, our method unleashes applications such as editing on real images, generation with partial sketches and strokes, and multi-domain multi-modal synthesis.

==> tex/tab-i2i-fid.tex <==
\begin{table}[h!]
    \centering
    \tabcolsep=0.15cm
    \footnotesize
    \caption{\textbf{Quantitative Comparisons with Unpaired I2I Methods.} We measure the FID and NIQE scores across various datasets. VQ-I2I performs comparably to the state-of-the-art methods on unpaired datasets, while enabling applications that cannot be done by these conventional I2I methods.}
    \label{tab:fid}
    \begin{tabular}{lcccccc} 
    \toprule
    dog$\rightarrow$cat & CycleGAN & DRIT & MUNIT & U-GAT-IT & CUT & \textbf{Ours} \\
    \midrule
     FID & 76.89 & 35.74 & 33.78 & 21.62 & 22.79 & xx.xx  \\
     NIQE & 40.65 & 47.32 & 63.64 & 59.84 & 48.95 & xx.xx \\
    
    % \multicolumn{1}{l}{} &  & CycleGAN & DRIT & MUNIT & U-GAT-IT & CUT & \textbf{Ours} \\
    % \multirow{2}{*}{dog-cat} & FID & 76.89 & 35.74 & 33.78 & 21.62 & 22.79 &  \\
    %  & NIQE & 40.65 & 47.32 & 63.64 & 59.84 & 48.95 &  \\
    \bottomrule
    \end{tabular}
% \vspace{-.5em}        
\end{table}
